In-Context Code-Text Learning for Bimodal Software Engineering

Bimodal software analysis initially appeared to be within reach with the advent of large language models. Unfortunately, the complex interplay of natural language text and code in software engineering, presents unique challenges that prevent pretrained models to generalize to a variety of tasks. We postulate that in-context learning for the code-text bimodality is a promising avenue. This paper thus introduces a comprehensive study of in-context code-text learning, focusing on leveraging pretrained CodeLLAMA models. We consider a diverse dataset encompassing 23 software engineering tasks, which we transform in an in-context learning format. To effectively extract informative features, we propose a configurable prompt template. Our proposed pipeline, InCTRL, then unifies prompt learning across various software engineering tasks. Extensive evaluation on the study datasets demonstrates the superiority of INCTRL-models in few-shot performance, surpassing state-of-the-art models including the support model, CodeLLAMA. Typically, we observe that applied to the CodeLLAMA model, INCTRL brings improvements in terms of precision (at least about 12\%) and recall (up to 93.88\%) on various tasks. For example, on the task of program repair, INCTRL improves the BLEU score of CodeLLAMA by 85 points, while for clone detection, INCTRL achieves an improvement of 69 percentage points. Moreover, INCTRL-models offer state-of-the-art performance when using retrieval-augmented generation on individual downstream tasks. Finally, we qualitatively analyze the benefits of INCTRL over CodeLLAMA and open-source all models for broader impact. We make our code and dataset publicly available at: \begin{center} {\url{https://anonymous.4open.science/r/inctrl-B65B}} \end{center}

==> macros1.tex <==
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% black text
\newcommand\black[1]{\textcolor{black}{#1}}
\usepackage{graphicx} % For including graphics
\usepackage{caption} % For captions
\usepackage{subcaption} % For subfigures
\usepackage{natbib}
\setcitestyle{numbers,square}
\usepackage{xspace}
\usepackage{booktabs}
\usepackage{moreverb}
\usepackage{fontenc}
\usepackage{amsmath}
\usepackage{fancybox}
\usepackage{color}
\usepackage{colortbl}
\usepackage{array}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{listings}
\usepackage{makecell}
\usepackage{graphicx}
\usepackage{setspace}
\usepackage[multiple]{footmisc}
\usepackage{wasysym}
\usepackage{balance}
\usepackage{csvsimple}
\usepackage{longtable}
\usepackage{caption}
\usepackage{url}
\usepackage{lscape}
\usepackage{rotating}
\usepackage{tikz}
\usepackage{enumitem}
\usepackage{subcaption}
\usepackage{marvosym}
\usepackage{pifont}% http://ctan.org/pkg/pifont%\usepackage{subfigure}
\usepackage{courier}
\usepackage{afterpage,lipsum}
\usepackage{booktabs}
\usepackage{threeparttable}
\usepackage{tcolorbox}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{float}
\usepackage{soul}
\usepackage{rotating} 




\lstset{
  frame=tb,
  framerule=0.2mm,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small\ttfamily},
%   numbers=left,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  escapeinside=``,
  tabsize=4,
  extendedchars=false
}


\lstset{
    basicstyle=\ttfamily,
    mathescape, % Allows $...$ to be treated as math mode in listings
    breaklines=true, % Allows line breaking
    postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space}
}


% variable definition
\newcommand{\tang}[1]{\textcolor{blue}{Tang: }\textcolor{red}{#1}}
\newcommand{\toolname}{\emph{\sc PatchRep}\xspace}

\newcommand{\basicalert}[2]{\fbox{\bfseries\sffamily\scriptsize\color{blue} #1}{\sf\small$\blacktriangleright$\textit{\color{red} #2}$\blacktriangleleft$}}
\newcommand{\jk}[1]{\basicalert{Jacques}{#1}}
\newcommand{\tb}[1]{\basicalert{Bissyande}{#1}}
\newcommand{\daniel}[1]{\basicalert{From Daniel}{#1}}
\newcommand{\tian}[1]{\basicalert{From Haoye}{#1}}
\newcommand{\yw}[1]{\basicalert{From Yewei}{#1}}
\newcommand{\ah}[1]{\basicalert{From Andrew}{#1}}
\newcommand{\ak}[1]{\basicalert{From Saad}{#1}}
\newcommand{\kisub}[1]{\basicalert{From Kisub}{#1}}


\newcommand{\definition}[1]{
	\setlength{\fboxrule}{1pt}
	\begin{center}\
		\noindent\fcolorbox{black}{white!10}{
			\begin{minipage}{.92\linewidth}
				#1
			\end{minipage}
		}
	\end{center}
	\smallskip
}

\newcommand{\find}[1]{
\begin{tcolorbox}[leftrule=0.4mm,rightrule=0mm,toprule=0mm,bottomrule=0mm,left=0.0pt,right=0.0pt,top=0pt,bottom=0pt]%[tile,size=fbox,boxsep=2mm,boxrule=0pt,top=0pt,bottom=0pt,borderline={0.5mm}{0pt}{black!70!white},colback=black!5!white]
\em #1
\end{tcolorbox}
}


% \newcommand{\find}[1]{
% 	\setlength{\fboxrule}{1pt}
% 	\begin{center}\
% 		\noindent\fcolorbox{black}{gray!10}{
% 		\begin{minipage}{.92\linewidth}
% 			#1
% 		\end{minipage}
% 	}
% 	\end{center}
% 	\smallskip
% }

\pagestyle{plain}

==> sections/Exps/tmp/RQ1.tex <==
\subsection{Overall performance of \toolname}
In this section, we evaluate the performance of \toolname and compare against the selected baselines across the PatchDB and SPI-DB datasets. 
Table~\ref{tab:comparison} reports the performance measurements on different metrics. 

\begin{table}[h!]
    \centering
    \caption{Performance metrics (\%) on security patch detection}
    \resizebox{\linewidth}{!}{
    \label{tab:comparison}
    \begin{tabular}{c|c|c|c|c|c}
        \hline

        \hline

        \hline

        \hline
       \bf Method & \bf Dataset & \bf AUC & \bf F1 & \bf +Recall & \bf -Recall \\
        \midrule
        \multirow{2}{*}{$\begin{array}{c}\text{TwinRNN} \\
        \text{\cite{wang2021patchrnn}}\end{array}$} & PatchDB & 66.50 & 45.12 & 46.35 & 54.37 \\
        & SPI-DB & 55.10 & 47.25 & 48.00 & 52.10  \\
        \hline 
        \multirow{2}{*}{$\begin{array}{c}\text{GraphSPD} \\
        \text{\cite{wang2023graphspd}}\end{array}$} & PatchDB & 78.29 & 54.73 & 75.17 & 79.67\\
        & SPI-DB & 63.04 & 48.42 & 60.29 & 65.33  \\
        \hline 
        \multirow{2}{*}{$\begin{array}{c}\text{GPT (v3.5)} \\
        \end{array}$} & PatchDB & 50.01 & 52.97 & 49.28 & 50.67\\
        & SPI-DB & 49.83 & 42.19 & 44.70 & 55.20  \\
        \hline 
        \multirow{2}{*}{$\begin{array}{c}\text{Vulfixminer~\cite{zhou2021finding}} \\
        \end{array}$} & PatchDB & 71.39 & 64.55 & 55.72 & 77.03 \\
        & SPI-DB & 68.04 & 54.42 & 68.14 & 62.04 \\
        \hline 
        \multirow{2}{*}{$\begin{array}{c}\text{CodeT5~\cite{wang2021codet5}} \\
        \end{array}$} & PatchDB & 71.00 & 63.73 & 54.98 & 76.18 \\
        & SPI-DB & 72.88 & 56.77 & 65.45 & 68.75 \\
        \hline
        \multirow{2}{*}{\textbf{LLMDA}} & PatchDB & \cellcolor{black!25}84.49 ($\pm$ 0.51) & \cellcolor{black!25}78.19 ($\pm$ 0.37) & \cellcolor{black!25}80.22 ($\pm$ 0.21) & \cellcolor{black!25}87.33 ($\pm$ 0.24) \\
        & SPI-DB & \cellcolor{black!25}68.98 ($\pm$ 0.27) & \cellcolor{black!25}58.13 ($\pm$ 0.33) & \cellcolor{black!25}70.94 ($\pm$ 0.13) & \cellcolor{black!25}80.62 ($\pm 0.22$)  \\
        \hline

        \hline

        \hline

        \hline
    \end{tabular}}
   % \vspace{-0.5cm}
\end{table}

\toolname is consistently able to identify security patches and recognize non-security patches. On the PatchDB dataset, this performance reaches 80\% and 87\%, respectively, for +Recall and -Recall. On the SPI-DB dataset, the performance is lower but, again, consistent across both classes. 

The results achieved by the baselines (cf. Table~\ref{tab:comparison}) further demonstrate the superior performance of \toolname. On the PatchDB dataset, \toolname significantly outperforms token-driven neural network approaches, including VulfixMiner, TwinRNN, and GPT 3.5 on all metrics. The performance improvement ranges from $\sim$18\% to $\sim$24\% in terms of AUC. This large improvement is also noticeable in the other metrics and with the SPI-DB dataset. 

With respect to the incumbent state-of-the-art, GraphSPD, we note that \toolname outperforms it by about 6, 23, 5, and 8 percentage points, respectively, in terms of AUC, F1, +Recall, and -Recall on the PatchDB dataset. On the SPI-DB dataset, the metric improvements are also substantial: 5 (AUC), 10 (F1), 10 (+Recall) and 15 (-Recall) percentage points.




% \daniel{should we directly remove the following?}
% Considering the inherent challenges associated with directly applying GPT3.5 for classification tasks, its comparative underperformance against specialized models like \toolname, TwinRNN, and GraphSPD becomes evident. GPT3.5's broad, general-purpose design, coupled with its lack of targeted domain knowledge, renders it less efficacious for nuanced classification objectives. The model's primary architecture, optimized for generating and understanding complex natural language across a wide range of topics, does not inherently focus on the specific patterns and distinguishing features critical for classification accuracy~\cite{shi2023chatgraph}\cite{reiss2023testing}. 
% % This discrepancy underscores the importance of leveraging models that are either intrinsically designed for or have been fine-tuned to excel in specific classification tasks, which can more adeptly identify and categorize the nuanced data points essential for high-performance outcomes in such applications.


% \begin{table}[h!]
%     \caption{Performance of \toolname without augmentation and instruction}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \label{tb:originaldataset}
%     \begin{tabular}{c|c|c|c|c|c}
%         \hline

%         \hline

%         \hline

%         \hline
%         Method & Dataset & AUC & F1 & +Recall & -Recall \\
%         \hline
%         \multirow{2}{*}{LLMDA} 
%         & PatchDB & 82.54 & 75.25 & 77.26 & 82.80  \\
%         & SPI-DB & 65.54 & 55.76 & 67.30 & 76.09  \\
%         \hline

%         \hline

%         \hline

%         \hline
%     \end{tabular}}
% \end{table}

% In exploring the advantages of \toolname, experiments were conducted on the original dataset without explanations from LLM and instructions, maintaining the same input size. Thus, the input consisted of \textbf{\texttt{<}patch, [CLS], description, [CLS]} \textbf{\texttt{>}} instead of \textbf{\texttt{<}patch, explanation, description, instruction} \textbf{\texttt{>}}. Despite the absence of explanations and instructions, \toolname consistently outperforms the state-of-the-art method, GraphSPD, across all metrics in Table~\ref{tb:originaldataset}. Notably, \toolname achieves a significant improvement compared to GraphSPD, with higher AUC, F1 score, positive recall, and negative recall. Specifically, on the PatchDB dataset, \toolname's performance shows an increase of approximately 5.43\% in AUC, 37.42\% in F1 score, 2.78\% in positive recall, and  3.93\% in negative recall compared to GraphSPD. Similarly, on the SPI-DB dataset, \toolname demonstrates superiority over GraphSPD, with improvement percentages of approximately 3.96\% in AUC, 15.18\% in F1 score, 11.63\% in positive recall, and 16.45\% in negative recall. These findings underscore \toolname's robustness in accurately distinguishing between security and non-security patches, even without additional explanations and instructions.

\find{{\bf  [RQ-1] \ding{42} } \toolname is effective in detecting security patches. With an F1 score at 78.19\%, \toolname demonstrates a well-balanced performance: our model can concurrently attain high precision and high recall. Specifically, we achieved a new state-of-the-art performance in identifying both security patches (+Recall) and recognizing non-security patches (-Recall). Comparison experiments further confirm that \toolname is superior to the baselines and is consistently high-performing across the datasets and across the metrics. 
}

% \find{{\bf RQ-1 Insights:}
% The comparative analysis underscores \toolname's superior performance in security patch detection across multiple evaluation metrics and datasets. Its consistent outperformance across varied metrics suggests that \toolname leverages a more effective methodology for analyzing patch data.}


==> sections/Exps/tmp/RQ2.tex <==
\subsection{Contributions of key design decisions} 
In this section we investigate the impact of key design choices on the overall performance of \toolname. To that end, we perform an ablation study on :
\begin{itemize}%[leftmargin=*]
    \item {\em Inputs}: Compared to prior works, \toolname innovates by considering two additional inputs, namely an LLM-generated explanation of the code changes as well as an instruction. What performance gain do we achieve thanks to these inputs? 
    \item {\em Representations:} A major contribution of the \toolname design is the {\em PT-Former} module, which enables to align and concatenate bimodal input representations belonging to different embedding spaces. What performance gap is filled by PT-Former?
    \item {\em Classifiers:} \toolname relies on stochastic batch contrastive learning to enhance its discriminative power, in particular for samples that are close to the decision boundaries of security relevance. To what extent does SBCL maximize \toolname's performance?
\end{itemize}

To answer the aforementioned sub-questions, we build variants of \toolname where different components are removed. We then compute the performance metrics of each variant and compare them against the original \toolname.

\subsubsection{\bf \em Impact of LLM-generated explanations}
We build a variant {\sc llmda}$_{EX-}$ where the explanation input is replaced by ``[CLS]''. Indeed, changing the PT-Former architecture to consider three inputs may bias the experiments. Instead, we follow the convention recognized by transformer-based models: the ``[CLS]'' token represents the classification token and is positioned at the beginning of the input sequence, serving as a signal for the model to generate a representation suitable for classification tasks. In our case, since the instruction input also indicates that the representation is for a classification task, our replacement has no side effect. 

{\sc llmda}$_{EX-}$ allows us to investigate the model's performance when the contextual information provided by the LLM-generated explanation is not provided. Table~\ref{tb:woex} reports the performance results that are achieved in this ablation study.

\begin{table}[h!]
    \caption{Performance (\%) of {\sc llmda}$_{EX-}$ (without the LLM-generated explanations)}
    \centering
    \resizebox{\linewidth}{!}{
    %\label{tab:ablationstudy}
    \begin{threeparttable}  
    \begin{tabular}{c|c|c|c|c|c}
        \hline

        \hline

        \hline

        \hline 
        Model & Dataset & AUC & F1 & +Recall & -Recall  \\
        \midrule
        \multirow{2}{*}{{\sc llmda}$_{EX-}$}
        & PatchDB & 83.24 (\textcolor{red}{$\downarrow1.25$})\tnote{$*$} & 76.73 (\textcolor{red}{$\downarrow1.46$})\tnote{$*$} & 79.01 & 86.09   \\
        & SPI-DB & 68.27 (\textcolor{red}{$\downarrow0.71$})\tnote{$*$} & 57.57 (\textcolor{red}{$\downarrow0.56$})\tnote{$*$} & 70.23 & 80.07  \\
        \hline

        \hline

        \hline

        \hline
    \end{tabular}
    \begin{tablenotes}
    \item[*] \textcolor{red}{($\downarrow x.xx$)} measures the performance drop when comparing against \toolname.
  \end{tablenotes}
    \end{threeparttable}}
    \label{tb:woex}
   % \vspace{-0.2cm}
\end{table}

 It is noticeable that the performance of {\sc llmda}$_{EX-}$ is consistently lower across the various metrics and across the datasets. These findings highlight the significance of LLM-generated explanations in enhancing the model's predictive capabilities.


\subsubsection{\bf \em Impact of instruction}
We conduct an ablation study based on a variant, {\sc llmda}$_{IN-}$, where the designed instruction is replaced with the ``[CLS]'' token as in the previous ablation study. The performance of this variant on the PatchDB and SPI-DB datasets is reported in Table~\ref{tb:woin}.

\begin{table}[h!]
    \caption{Performance (\%) of {\sc llmda}$_{IN-}$ (without the designed instruction)}
    \centering
    \resizebox{\linewidth}{!}{
    \label{tab:ablationstudy}
    \begin{tabular}{c|c|c|c|c|c}
        \hline

        \hline

        \hline

        \hline 
        Model & Dataset & AUC & F1 & +Recall & -Recall \\
        \midrule
        \multirow{2}{*}{\sc llmda$_{IN-}$} 
        & PatchDB & 82.51 (\textcolor{red}{$\downarrow 1.98$}) & 76.14 (\textcolor{red}{$\downarrow 2.05$}) & 78.55 & 85.64   \\
        & SPI-DB & 67.93 (\textcolor{red}{$\downarrow 1.05$}) & 57.25 (\textcolor{red}{$\downarrow 0.88$}) & 69.90 & 79.62  \\
        \hline

        \hline

        \hline

        \hline
    \end{tabular}}
    \label{tb:woin}
    %\vspace{-0.2cm}
\end{table}

Again, we note that the performance drops compared to \toolname. It even appears that, without the instruction, the performance drop is slightly more important than when the model does not include the LLM-generated explanations. These findings underscore the importance of the label-wise design decision based on explicitly adding an instruction among the inputs for embedding to enhance the model's performance for security patch detection.

\subsubsection{\bf \em Impact of PT-Former}
To investigate the importance of {\em PT-Former}, we design a variant,  {\sc llmda}$_{PT-}$ where the {\em PT-Former} space alignment \& representation combination module is removed. To that end, we must still design some simple computations to generate one embedding space for all inputs. In our case, the embeddings of the code and text input tokens have the same dimension ($768$). We thus concatenate them:
\begin{equation}
E = \mathrm{Avg}(E_{p}+E_{expl}) \oplus E_{desc} \oplus E_{inst}
\end{equation}

where $\mathrm{Avg}$ is the average operation and $\oplus$ is the concatenation operation.

\begin{table}[h!]
    \caption{Performance (\%) of {\sc llmda$_{PT-}$} (without the {\em PT-Former} module)}
    \centering
    \resizebox{\linewidth}{!}{
    \label{tab:ablationstudy}
    \begin{tabular}{c|c|c|c|c|c}
        \hline

        \hline

        \hline

        \hline 
        Model & Dataset & AUC & F1 & +Recall & -Recall  \\
        \midrule
        \multirow{2}{*}{\sc llmda$_{PT-}$} 
        & PatchDB & 80.36 (\textcolor{red}{$\downarrow 4.13$}) & 70.24 (\textcolor{red}{$\downarrow 7.95$}) & 69.54 & 83.18  \\
        & SPI-DB & 63.17 (\textcolor{red}{$\downarrow 5.81$}) & 54.62 (\textcolor{red}{$\downarrow 3.51$})& 67.15 & 73.51   \\
        \hline

        \hline

        \hline

        \hline
    \end{tabular}}
    \label{tb:wopt}
    \vspace{-0.2cm}
\end{table}


The performance results of {\sc llmda$_PT-$} are reported in Table~\ref{tb:wopt}. Compared to other variants of \toolname, {\sc llmda$_{PT-}$} achieves the lowest scores across all evaluated metrics. On PatchDB, compared to the original \toolname, {\sc llmda$_{PT-}$} performance is dropped by 4.13\%, 7.95\% in terms of AUC and F1. Actually, {\sc llmda$_{PT-}$} has over 10\% less +Recall, meaning that it is significantly under-performing in the task of identifying security patches. On SPI-DB, the performance gap is larger on -Recall (it fails to recognize non-security patches). These findings confirm that the design decisions in {PT-Former} have been instrumental to the performance of \toolname.

\subsubsection{\bf \em Impact of SBCL}
In \toolname we designed SBCL to optimize the model's ability to discern different patterns between positive (security patches) and negative (non-security patches) examples more effectively.  Figure~\ref{fig:sbclwo} illustrates the ambition: after PT-Former learns the representations, the embedding subspaces of security and non-security patches will certainly intersect on some ``difficult'' samples. SBCL is designed to find the optimum decision boundary. 
To assess the importance of SBCL, we design a variant, {\sc llmda$_{SBCL-}$}, where we directly feed the embeddings processed by \textit{PT-Former} into the fully connected layer (i.e., without the stochastic batch contrastive learning step).%  as shown in Figure~\ref{fig:sbcl}.

\begin{figure}[ht]
    \vspace{-0.5cm}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/sbcl-01.pdf}
    \caption{Illustration of embedding subspaces of security/non-security patches for contrastive learning}
    \label{fig:sbclwo}
    \vspace{-0.2cm}
\end{figure}

Table~\ref{tb:wosbcl} presents the performance results of {\sc llmda$_{SBCL-}$}. Compared to the original \toolname, the performance drop is noticeable. Despite the relatively small proportion of the semantic space at the intersection between the subspaces of security and non-security patches, SBCL enables to achieve 1-3 percentage points improvement on the different metrics.

\begin{table}[h!]
    \caption{Performance (\%) of {\sc llmda$_{SBCL-}$} (without contrastive learning)}
    \centering
    \resizebox{\linewidth}{!}{
    \label{tab:ablationstudy}
    \begin{tabular}{c|c|c|c|c|c}
        \hline

        \hline

        \hline

        \hline 
        Model & Dataset & AUC & F1 & +Recall & -Recall   \\
        \midrule
        \multirow{2}{*}{\sc llmda$_{SBCL-}$} 
        & PatchDB & 82.93 (\textcolor{red}{$\downarrow 1.56$}) & 76.45 (\textcolor{red}{$\downarrow 1.74$}) & 78.72 & 85.81  \\
        & SPI-DB & 67.43 (\textcolor{red}{$\downarrow 1.55$}) & 56.61 (\textcolor{red}{$\downarrow 1.52$}) & 69.45 & 79.10 \\
        \hline

        \hline

        \hline

        \hline
    \end{tabular}}
    \label{tb:wosbcl}
\end{table}
%\daniel{In our analysis of 967 complex cases in PatchDB to compare the performance of \toolname and GraphSPD, particularly in scenarios known to challenge both tools, \toolname accurately identified 724 cases, showing a slightly higher precision than GraphSPD, which accurately predicted 709 cases. This indicates that \toolname has a marginally better capability in handling hard samples.}

% Furthermore, the utilization of SBCL enables the model to learn more discriminative features and better capture the underlying characteristics of the data, resulting in improved classification performance. These findings underscore the importance of incorporating SBCL as a training strategy to optimize the performance of models in security patch classification tasks.





\find{{\bf  [RQ-2] \ding{42} }
The ablation study results reveal that each of the key design decisions contributes noticeably to the performance of \toolname. In particular, without the {\em PT-Former} module \toolname would lose about 8 percentage points in F1. 
%LLM-generated explanations, SBCL as well as the instruction are each individually important components.
}



==> sections/Exps/tmp/RQ3.tex <==
\subsection{Discriminative power of \toolname representations}\label{sec:type}
In this section, we investigate to what extent the representations obtained with \toolname are indeed enabling a good separation of security and non-security patches in the embedding space. To that end, we consider two separate evaluations: the first attempts to visualize the embedding space of \toolname and compares it against the one of GraphSPD (i.e., the state of the art); the second qualitatively assesses two case studies.

\subsubsection{\bf \em Visualization of embedding spaces}
We consider 1\,000 random patches from our PatchDB dataset. We then collect their associated embeddings from \toolname and GraphSPD and apply principal component analysis (PCA)~\cite{smith2002tutorial}. Given the imbalance of the dataset, the drawn samples are largely non-security patches, while security patches are fewer. Figure~\ref{fig:visual} presents the PCA visualizations of the representations.

\begin{figure}[!h]
    %\vspace{-0.2cm}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
    \centering
        \includegraphics[width=0.75\columnwidth]{figures/graphspdv.pdf}
        \caption{Embeddings yielded by GraphSPD}
        \label{fig:sub1}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=0.75\columnwidth]{figures/llmdav.pdf}
        \caption{Embeddings yielded by \toolname}
        \label{fig:sub2}
    \end{subfigure}
    \caption{PCA visualizations of security and non-security patch embeddings by GraphsSPDand \toolname.
    }
    \label{fig:visual}
    %\vspace{-0.2cm}
\end{figure}
 
\begin{table*}[!t]
    \centering
    \caption{Attention scores for security and non-security labels by GraphSPD and \toolname on two sample patches}
    \resizebox{1\linewidth}{!}{
\begin{tabular}{>{\centering}m{0.4\linewidth}|m{0.2\linewidth}|>{\centering}m{0.4\linewidth}|m{0.2\linewidth}|m{0.2\linewidth}}
\hline

\hline

\hline

\hline

\multicolumn{2}{c|}{GraphSPD (failed cases)} & \multicolumn{3}{c}{\toolname (successful cases)} \\
    \cline{1-5}
 Patch ({\em non-formatted token sequence}) & Developer Description& Patch ({\em non-formatted token sequence})& Explanation & Description \\ \hline
 
\scriptsize \tt diff --git a/sgminer.c b/sgminer.cindex a7dd3ab3..08697cd0 100644--- a/sgminer.c+++ b/sgminer.c@@ -518,7 +518,7 @@ struct pool \textcolor{red}{*add\_pool(void)}\textcolor{blue}{ \rm \em  \textbf{(non-security score = 0.65)}}sprintf(buf, "Pool \%d", pool\texttt{->}\_no);pool\texttt{->}poolname = strdup(buf);-\textbackslash tpools = realloc(pools, sizeof(struct pool *) \*(total\_pools + 2));+\textbackslash tpools = (struct **pool **)realloc(pools, sizeof(struct pool *) * (total\_pools + 2));pools[total\_pools++] = pool;mutex\_init(\&pool\texttt{->}pool\_lock); if(unlikely({pthread\_cond\_init}(\&pool\texttt{->}cr\_cond, NULL))) 
& Fixed missing realloc removed by mistake & \scriptsize \tt diff --git a/sgminer.c b/sgminer.cindex a7dd3ab3..08697cd0 100644--- a/sgminer.c+++ b/sgminer.c@@ -518,7 +518,7 @@ struct pool *add\_pool(void)sprintf(buf, "Pool \%d", pool\texttt{->}\_no);pool\texttt{->}poolname = strdup(buf);-\textbackslash tpools = \textcolor{red}{\textbf{realloc(pools, sizeof(struct pool *) \*(total\_pools + 2));+\textbackslash tpools = (struct **pool **)realloc(pools, sizeof(struct pool *) * (total\_pools + 2));}} \textcolor{blue}{\rm \em \textbf{(security core = 0.57)}} pools[total\_pools++] = pool;\textcolor{red}{\textbf{mutex\_init}}\textcolor{blue}{\rm \em \textbf{(security core = 0.50)}}(\&pool\texttt{->}pool\_lock); if(unlikely({pthread\_cond\_init}(\&pool\texttt{->}cr\_cond, NULL)))  & Modified sgminer.c, adjusted \textcolor{red}{\textbf{realloc usage}}\textcolor{blue}{\rm \em \textbf{(security core = 0.67)}} with \textcolor{red}{\textbf{explicit type casting}}\textcolor{blue}{\rm \em \textbf{(security core = 0.63)}} & Fixed missing \textcolor{red}{\textbf{realloc}}\textcolor{blue}{\rm \em 
 \textbf{(security core = 0.63)}} removed by mistake\\ 
\hline

\hline

\hline

\hline

\scriptsize \tt diff --git a/lib/krb5/auth\_context.c b/lib/krb5/auth\_context.c index 0edea5418..3cba484e1 100644 --- a/lib/krb5/auth\_context.c +++ b/lib/krb5/auth\_context.c @@ -53,6 +53,7 @@ \textcolor{red}{\textbf{krb5\_auth\_con\_init}}\textcolor{blue}{\rm \em \textbf{(non-security score = 0.60)}}(krb5\_context context, \textcolor{red}{\textbf{ALLOC}}\textcolor{blue}{\rm \em 
 \textbf{(non-security score = 0.67)}}(p\texttt{->}authenticator, 1); if (!p\texttt{->}authenticator) return ENOMEM; +    memset (p\texttt{->}authenticator, 0, sizeof(*p\texttt{->}authenticator)); p\texttt{->}flags = KRB5\_AUTH\_CONTEXT\_DO\_TIME; 
& zero authenticator
& \scriptsize \tt diff --git a/lib/krb5/auth\_context.c b/lib/krb5/auth\_context.c index 0edea5418..3cba484e1 100644 --- a/lib/krb5/auth\_context.c +++ b/lib/krb5/auth\_context.c @@ -53,6 +53,7 @@ krb5\_auth\_con\_init(krb5\_context context, ALLOC(p\texttt{->}authenticator, 1); if (!p\texttt{->}authenticator) return ENOMEM; +    \textcolor{red}{\textbf{memset (p\texttt{->}authenticator, 0, sizeof(*p\texttt{->}authenticator));}}\textcolor{blue}{\rm \em \textbf{(security core = 0.59)}} p\texttt{->}flags = KRB5\_AUTH\_CONTEXT\_DO\_TIME; 
& Added
memset to initialize \textcolor{red}{\textbf{`authenticator' memory in krb5\_auth\_
con\_init function}}\textcolor{blue}{\rm \em \textbf{(security core = 0.84)}}. & \textcolor{red}{\textbf{zero authenticator}} \textcolor{blue}{\rm \em \textbf{(security core = 0.77)}}\\
\hline

\hline

\hline

\hline
\end{tabular}}
    \label{tb:case}
\end{table*}

 We observe from the distribution of data points that  \toolname can effectively separate the two categories (i.e., security and non-security patches), in contrast to the incumbent state-of-the-art, GraphSPD. This finding suggests that the representations of \toolname are highly relevant for the task of security patch detection. 
%  \url{llmda.github.io}.


==> sections/Exps/tmp/RQ4.tex <==
\subsubsection{\bf \em Case studies}
Table~\ref{tb:case} presents 2 examples to illustrate the difference between \toolname and GraphSPD in terms of what the representations can capture, and potentially explaining why \toolname was successful on these cases while GraphSPD was not. For our classification task, we have two labels: security (0) and non-security (1). 
For \toolname, we can directly consider the label name in the instruction. Thus we compute the attention map between security and the tokens in the patch, the explanation, and the description. For  GraphSPD, however, since there no real label name involved in the training and inference phases, we compute the attention score between the words in the patch and the number ``0" or ``1". 
To simplify the analysis, we only highlight, in Table~\ref{tb:case}, tokens for which the similarity score is higher than 0.5.

As shown in the examples, \toolname generally assigns high similarity scores to security-related aspects, suggesting a detection capability that nuances between tokens. For example, in the sgminer.c patch, \toolname gives high scores to \textit{realloc} and \textit{mutex\_init}, indicating a finer sensitivity to potential security implications within these code parts. Similarly, in the krb5/auth\_context.c patch, the use of \textit{memset} for initializing authenticator memory is scored high in \toolname, reflecting its more acute recognition of security practices.

In contrast, since GraphSPD is graph-based, it focuses on the patch itself. For the same patch cases, GraphSPD can even give  very high attention scores for non-security label. For example, \textit{krb5\_auth\_con\_init} is given 0.6 score for ``non-security" and \textit{ALLOC} is given 0.67 attention score towards non-security as well. These scores may justify many failures of GraphSPD in the security patch detection task.

% \begin{table*}[!t]
%     \centering
%     \caption{Attention scores for security and non-security labels by GraphSPD and \toolname on two sample patches}
%     \resizebox{1\linewidth}{!}{
% \begin{tabular}{>{\centering}m{0.4\linewidth}|m{0.2\linewidth}|>{\centering}m{0.4\linewidth}|m{0.2\linewidth}|m{0.2\linewidth}}
% \hline

% \hline

% \hline

% \hline

% \multicolumn{2}{c|}{GraphSPD (failed cases)} & \multicolumn{3}{c}{\toolname (successful cases)} \\
%     \cline{1-5}
%  Patch  & Description& Patch & Explanation & Description \\ \hline
 
% diff --git a/sgminer.c b/sgminer.cindex a7dd3ab3..08697cd0 100644--- a/sgminer.c+++ b/sgminer.c@@ -518,7 +518,7 @@ struct pool \textcolor{red}{*add\_pool(void)}\textcolor{blue}{\textbf{(non-security score =0.65)}}sprintf(buf, "Pool \%d", pool\texttt{->}\_no);pool\texttt{->}poolname = strdup(buf);-\textbackslash tpools = realloc(pools, sizeof(struct pool *) \*(total\_pools + 2));+\textbackslash tpools = (struct **pool **)realloc(pools, sizeof(struct pool *) * (total\_pools + 2));pools[total\_pools++] = pool;mutex\_init(\&pool\texttt{->}pool\_lock); if(unlikely({pthread\_cond\_init}(\&pool\texttt{->}cr\_cond, NULL))) 
% & Fixed missing realloc removed by mistake &diff --git a/sgminer.c b/sgminer.cindex a7dd3ab3..08697cd0 100644--- a/sgminer.c+++ b/sgminer.c@@ -518,7 +518,7 @@ struct pool *add\_pool(void)sprintf(buf, "Pool \%d", pool\texttt{->}\_no);pool\texttt{->}poolname = strdup(buf);-\textbackslash tpools = \textcolor{red}{\textbf{realloc(pools, sizeof(struct pool *) \*(total\_pools + 2));+\textbackslash tpools = (struct **pool **)realloc(pools, sizeof(struct pool *) * (total\_pools + 2));}} \textcolor{blue}{\textbf{(security core =0.57)}} pools[total\_pools++] = pool;\textcolor{red}{\textbf{mutex\_init}}\textcolor{blue}{\textbf{(security core =0.50)}}(\&pool\texttt{->}pool\_lock); if(unlikely({pthread\_cond\_init}(\&pool\texttt{->}cr\_cond, NULL)))  & Modified sgminer.c, adjusted \textcolor{red}{\textbf{realloc usage}}\textcolor{blue}{\textbf{(security core =0.67)}} with \textcolor{red}{\textbf{explicit type casting}}\textcolor{blue}{\textbf{(security core =0.63)}} & Fixed missing \textcolor{red}{\textbf{realloc}}\textcolor{blue}{\textbf{(security core =0.63)}} removed by mistake\\ 
% \hline

% \hline

% \hline

% \hline

% diff --git a/lib/krb5/auth\_context.c b/lib/krb5/auth\_context.c index 0edea5418..3cba484e1 100644 --- a/lib/krb5/auth\_context.c +++ b/lib/krb5/auth\_context.c @@ -53,6 +53,7 @@ \textcolor{red}{\textbf{krb5\_auth\_con\_init}}\textcolor{blue}{\textbf{(non-security score =0.60)}}(krb5\_context context, \textcolor{red}{\textbf{ALLOC}}\textcolor{blue}{\textbf{(non-security score =0.67)}}(p\texttt{->}authenticator, 1); if (!p\texttt{->}authenticator) return ENOMEM; +    memset (p\texttt{->}authenticator, 0, sizeof(*p\texttt{->}authenticator)); p\texttt{->}flags = KRB5\_AUTH\_CONTEXT\_DO\_TIME; 
% & zero authenticator
% &diff --git a/lib/krb5/auth\_context.c b/lib/krb5/auth\_context.c index 0edea5418..3cba484e1 100644 --- a/lib/krb5/auth\_context.c +++ b/lib/krb5/auth\_context.c @@ -53,6 +53,7 @@ krb5\_auth\_con\_init(krb5\_context context, ALLOC(p\texttt{->}authenticator, 1); if (!p\texttt{->}authenticator) return ENOMEM; +    \textcolor{red}{\textbf{memset (p\texttt{->}authenticator, 0, sizeof(*p\texttt{->}authenticator));}}\textcolor{blue}{\textbf{(security core =0.59)}} p\texttt{->}flags = KRB5\_AUTH\_CONTEXT\_DO\_TIME; 
% & Added
% memset to initialize \textcolor{red}{\textbf{`authenticator' memory in krb5\_auth\_
% con\_init function}}\textcolor{blue}{\textbf{(security core =0.84)}}. & \textcolor{red}{\textbf{zero authenticator}} \textcolor{blue}{\textbf{(security core =0.77)}}\\
% \hline

% \hline

% \hline

% \hline
% \end{tabular}}
%     \label{tb:case}
% \end{table*}




\find{{\bf  [RQ-3] \ding{42} }
The design of \toolname leads to patch representations that enable enhanced ability over GraphSPD in effectively differentiating between security and non-security patches on the embedding spaces. 
Our analysis of sample cases shows that \toolname assigns high attention scores to tokens associated to security-related aspects, making it effective for accurately identifying security patches.}


%and compare it with the state-of-the-art: GraphSPD.



% \subsection{Prompt Effect Study}




% \subsection{Supplementary Experiment}
% \subsubsection{Effect of Prompt for Patch Explanation}
% \subsubsection{Effect of Instruction}

==> sections/Exps/tmp/RQ5.tex <==
\subsection{Robustness of \toolname} 
A model is accepted as robust if it performs strongly on datasets that differ from the training data. For our study task, robustness should ensure reliable predictions on unseen patches. We assess the  
robustness of \toolname and GraphSPD by training them against the PatchDB and testing against the samples from the FFmpeg dataset used to construct the benchmark for Devign~\cite{zhou2019devign} vulnerability detector. This test data includes 13,962 data points, consisting of 8,000 security-related and 5,962 non-security-related parches. The selection of the FFmpeg dataset is motivated by its coverage of a wide range of vulnerabilities.

\begin{table}[htbp]
    \centering
    \caption{Performance (\%) of GraphSPD and \toolname against unseen patches from the FFmpeg dataset~\cite{zhou2019devign}. \newline {\scriptsize Numbers between parentheses ($\downarrow$X) corresponds to the drop of performance when compared to the evaluation in cross-validation with PatchDB}}
    \resizebox{\linewidth}{!}{
    \label{tb:robustness}
    \begin{threeparttable}
 
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \hline

        \hline

        \hline

        \hline
        Method & Accuracy & Precision & AUC & Recall & +Recall & -Recall & F1 \\
        \midrule
        GraphSPD & 43.65 & 51.15 & 44.81 & 36.88 & 36.88 (\textcolor{red}{$\mathbf{\downarrow}$\bf 38.29}) & 52.75 & 42.86 (\textcolor{red}{$\downarrow$\bf 11.74)}\\ \hline
        \toolname & \cellcolor{black!25}66.78 & \cellcolor{black!25}72.70 & \cellcolor{black!25}66.69 & \cellcolor{black!25}67.30 & \cellcolor{black!25}67.30 (\textcolor{red}{$\downarrow$12.92}) & \cellcolor{black!25}66.09 & \cellcolor{black!25}69.89 (\textcolor{red}{$\downarrow$8.3})\\
        \hline

        \hline

        \hline

        \hline
    \end{tabular}
         \begin{tablenotes}
    \item[*] (\textcolor{red}{$\downarrow x.xx$}) measures the performance drop when comparing with the cross-validation of \toolname on Patch-DB (cf. Table~\ref{tab:comparison}).
  \end{tablenotes}      
    \end{threeparttable}
    }
\end{table}




Table~\ref{tb:robustness} summarizes the performance results of  \toolname and GraphSPD on the unseen dataset. Overall, on all metrics, \toolname exhibits a significantly superior performance  over GraphSPD, with about 20 percentage points of gap in terms of precision for example. We further highlight in the results the performance decrease between the test on unseen data and the cross-validation test in terms of F1 and +Recall (i.e., the ability to identify security patches). We note that the robustness of \toolname is substantially higher than GraphSPD:  GraphSPD loses about 38 percentage points of +Recall when \toolname only loses about 13 points. 


\find{{\bf  [RQ-4] \ding{42} }
Experiments on unseen patches clearly demonstrate that \toolname is more robust than GraphSPD. In terms of the ability to identify security patches, GraphSPD performance is dropped about threefold compared to \toolname under the same experimental settings.}





==> sections/appendices.tex <==
\appendices{}

\section{Datasets}
\label{appendix_datasets}

In Table~\ref{detailed_datasets}, we provide detailed information about all the datasets involved in the experiments of this work. The datasets can be downloaded using the Huggingface download interface and the corresponding repository IDs. It is worth noting that for some datasets, we only used a subset, which is indicated in the ``Remark'' column.

\begin{table*}[ht]

\centering
\captionsetup{justification=centering}
\caption{Detailed information of datasets involved in this work.}

\resizebox{.95\linewidth}{!}{
\begin{tabular}
{
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l }
\hline
{\color[HTML]{000000} \textbf{Task}}                                                     & {\color[HTML]{000000} \textbf{Dataset}}  & {\color[HTML]{000000} \textbf{Huggingface Repository ID}}                     & {\color[HTML]{000000} \textbf{Remark}}              \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} Big-Vul}           & {\color[HTML]{000000} benjis/bigvul}                                          & {\color[HTML]{000000} }                             \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} Draper}            & {\color[HTML]{000000} claudios/Draper}                                        & {\color[HTML]{000000} }                             \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} D2A}               & {\color[HTML]{000000} claudios/D2A}                                           & {\color[HTML]{000000} subset=``function''}          \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} ReVeal}            & {\color[HTML]{000000} claudios/ReVeal}                                        & {\color[HTML]{000000} }                             \\
\multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Vulnerability Detection}} & {\color[HTML]{000000} Devign}            & {\color[HTML]{000000} code\_x\_glue\_cc\_defect\_detection}                   & {\color[HTML]{000000} }                             \\ \hline
{\color[HTML]{000000} Clone Detection}                                                   & {\color[HTML]{000000} BigCloneBench}     & {\color[HTML]{000000} code\_x\_glue\_cc\_clone\_detection\_big\_clone\_bench} & {\color[HTML]{000000} }                             \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} InstructHumanEval} & {\color[HTML]{000000} codeparrot/instructhumaneval}                           & {\color[HTML]{000000} }                             \\
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Code Completion}}         & {\color[HTML]{000000} Safim}             & {\color[HTML]{000000} gonglinyuan/safim}                                      & {\color[HTML]{000000} }                             \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} CodeXGLUE}         & {\color[HTML]{000000} code\_x\_glue\_cc\_code\_to\_code\_trans}               & {\color[HTML]{000000} }                             \\
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Code Translation}}        & {\color[HTML]{000000} HumanEval-X}       & {\color[HTML]{000000} THUDM/humaneval-x}                                      & {\color[HTML]{000000} java-to-python}               \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} CodeXGLUE}         & {\color[HTML]{000000} ayeshgk/code\_x\_glue\_cc\_code\_refinement\_annotated} & {\color[HTML]{000000} }                             \\
\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Program Repair}}          & {\color[HTML]{000000} HumanEvalPack}     & {\color[HTML]{000000} bigcode/humanevalpack}                                  & {\color[HTML]{000000} subset=``python''}            \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} CodeXGLUE}         & {\color[HTML]{000000} code\_x\_glue\_ct\_code\_to\_text}                      & {\color[HTML]{000000} subset=``java''}              \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} XLCoST}            & {\color[HTML]{000000} codeparrot/xlcost-text-to-code}                         & {\color[HTML]{000000} subset=``C++-program-level''} \\
\multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Code Summarization}}      & {\color[HTML]{000000} Funcom}            & {\color[HTML]{000000} apcl/funcom-java-long}                                  & {\color[HTML]{000000} }                             \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} APPS}              & {\color[HTML]{000000} codeparrot/apps}                                        & {\color[HTML]{000000} difficulties=``all''}         \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} MBPP}              & {\color[HTML]{000000} mbpp}                                                   & {\color[HTML]{000000} subset=``sanitized''}         \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} Mercury}           & {\color[HTML]{000000} Elfsong/Mercury}                                        & {\color[HTML]{000000} }                             \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} InstructHumanEval} & {\color[HTML]{000000} codeparrot/instructhumaneval}                           & {\color[HTML]{000000} }                             \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} StudentEval}       & {\color[HTML]{000000} wellesley-easel/StudentEval}                            & {\color[HTML]{000000} }                             \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} XLCoST}            & {\color[HTML]{000000} codeparrot/xlcost-text-to-code}                         & {\color[HTML]{000000} subset=``C++-program-level''} \\
\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} }                                          & {\color[HTML]{000000} CoNaLa}            & {\color[HTML]{000000} neulab/conala}                                          & {\color[HTML]{000000} subset=``curated''}           \\
\multirow{-8}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} Code Generation}}         & {\color[HTML]{000000} CONCODE}           & {\color[HTML]{000000} AhmedSSoliman/CodeXGLUE-CONCODE}                        & {\color[HTML]{000000} }                             \\ \hline
\end{tabular}}

\label{detailed_datasets}
\end{table*}
